An Effective Transition-based Model for Discontinuous NER

Unlike widely used Named Entity Recognition (NER) data sets in generic domains, biomedical NER data sets often contain mentions consisting of discontinuous spans. Conventional sequence tagging techniques encode Markov assumptions that are efficient but preclude recovery of these mentions. We propose a simple, effective transition-based model with generic neural encoding for discontinuous NER. Through extensive experiments on three biomedical data sets, we show that our model can effectively recognize discontinuous mentions without sacrificing the accuracy on continuous mentions.

==> TODO.tex <==
\subsection{The difference between nested mentions and overlapping mentions}



\subsection{Why the performance on ShARe is better than the one on CADEC.}
\begin{itemize}
    \item Entity type: ADE is more ambiguous than disorder
    \item Data set size: CADEC is smaller than other two ShARe data sets
    \item Length of mentions: mentions in CADEC are longer than the ones in ShARe
    \item Vocabulary richessness:  as the richness of the vocabulary increases, small amounts of text – such as the training data – become less representative of the full domain, causing performance to decrease. CADEC has higher term variations.
\end{itemize}

\begin{itemize}
    \item Positional encoding
    \item Label smoothing
    \item Teaching force
    \item Coordination Boundary Prediction~\cite{Ficler:Goldberg:EMNLP:2016}
    \item Dynamic oracle
    \item SemEval / CYP450
\end{itemize}

\section{Supplemental Material}

\begin{table*}[h]
\begin{small}
    \centering
    \begin{tabular}{r|l}
    \hline
    Sentence & Walked like that for about six months with increasing pain , especially in right thigh which felt . \\
    Gold mentions & 1. \textbf{pain in right thigh} \\
    Predictions & 1. \textcolor{blue}{pain} -- BIO Ext \\
    & -- Hyper G \\
    & 1. \textcolor{blue}{increasing pain} -- Our model \\ \hline
    Sentence & Stated with joint and pain and muscle weakness , depression , fatigue and cramps . \\
    Gold mentions & 1. \textbf{joint pain}; 2. \textit{muscle weakness}; 3. \textit{depression}; 4. \textit{fatigue}; 5. \textit{cramps} \\
    Predictions & 1. \textcolor{blue}{joint and pain}; 2. \textcolor{red}{muscle weakness}; 3. \textcolor{red}{depression}; 4. \textcolor{red}{fatigue}; 5. \textcolor{red}{cramps} -- BIO Ext \\
    & -- Hyper G \\
    & 1. \textcolor{red}{muscle weakness}; 2. \textcolor{blue}{pain weakness}; 3. \textcolor{blue}{joint weakness}; 4. \textcolor{red}{depression}; 5. \textcolor{red}{fatigue}; 6. \textcolor{red}{cramps} -- Our model \\ \hline
    Sentence & stopped taking them 4 years ago and still suffer terrible muscle pain and wasting . \\
    Gold mentions & 1. \textit{muscle pain}; 2. \textbf{muscle wasting} \\
    Predictions & 1. \textcolor{blue}{terrible muscle pain}; 2. \textcolor{blue}{wasting} -- BIO Ext \\
    & -- Hyper G \\
    & 1. \textcolor{red}{muscle pain}; 2. \textcolor{blue}{wasting} -- Our model \\ \hline
    Sentence & Then I sated having hip / leg / foot pain and numbness . \\
    Gold mentions & 1. \textbf{hip pain}; 2. \textbf{leg pain}; 3. \textit{foot pain}; 4. \textit{numbness} \\
    Predictions & 1. \textcolor{red}{foot pain}; 2. \textcolor{blue}{pain}; 3. \textcolor{red}{numbness} -- BIO Ext \\
    & -- Hyper G \\
    & 1. \textcolor{blue}{stated}; 2. \textcolor{red}{hip pain}; 3. \textcolor{red}{leg pain}; 4. \textcolor{red}{foot pain}; 5. \textcolor{red}{numbness} -- Our model \\ \hline
    Sentence & Severe joint pain in the shoulders and knees . \\
    Gold mentions & 1. \textit{Severe joint pain in the shoulders}; 2. \textit{Severe joint pain in the knees} \\
    Predictions & 1. \textcolor{blue}{Severe joint pain in the}; 2. \textcolor{red}{Severe joint pain in the knees} -- BIO Ext \\
    & None -- Hyper G \\
    & 1. \textcolor{red}{Severe joint pain in the shoulders}; 2. \textcolor{red}{Severe joint pain in the knees} -- Our model \\ \hline
    %Sentence & lots of pain in the muscles there , very tight . \\
    %Gold mentions & 1. \textit{lots of pain in the muscles}; 2. \textbf{muscles very tight} \\
    %Predictions & 1. \textcolor{blue}{lots of pain in the muscles there} -- BIO Ext \\
    %& None -- Hyper G \\
    %& 1. \textcolor{blue}{pain in the muscles} -- Our method \\ \hline
    Sentence & Joint and Muscle Pain / Stiffness .  \\
    Gold mentions & 1. \textbf{Joint pain}; 2. \textbf{Muscle Stiffness}; 3. \textit{Muscle Pain}; 4. \textbf{Joint Stiffness} \\
    Predictions & 1. \textcolor{blue}{Joint}; 2. \textcolor{red}{Muscle Pain}; 3. \textcolor{blue}{Stiffness} -- BIO Ext \\
    & 1. \textcolor{red}{Joint pain}; 2. \textcolor{blue}{Muscle Pain / Stiffness}; 3. \textcolor{blue}{Stiffness} -- Hyper G \\
    & 1. \textcolor{red}{Joint pain}; 2. \textcolor{red}{Muscle Pain}; 3. \textcolor{blue}{Stiffness} -- Our method \\ \hline
    \end{tabular}
\end{small}
    \caption{Example sentences involving discontiguous entities and predictions using different methods. These examples are taken from CADEC. Discontiguous entities are highlighted in bold, and correct predictions are highlighted in red, incorrect ones in blue.}
\end{table*}

==> figure2-hypergraph.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.45\textwidth]{figure2-hypergraph.pdf}
    \caption{A sub-hypergraph encoding two mentions within one sentence: \textit{`muscle pain'} and \textit{`muscle fatigue'}. The path representing discontinuous mention \textit{`muscle fatigue'} is: \textbf{A, E, T} nodes corresponding to token \textit{`muscle'}, \textbf{B}$_0$, two \textbf{O}$_1$, \textbf{B}$_1$ and \textbf{X} nodes. Subscripts of \textbf{B}$_0$ and \textbf{O}$_1$ are used to indicate the index of components or intervals within the mention.~\label{figure2-hypergraph}}
\end{figure}

==> table1-example.tex <==
\begin{table*}[tb]
    \centering
    \begin{tabular}{m{3.5cm}|m{8cm}|m{4cm}}
    \toprule
    \bf Scenarios & \bf Example sentence & \bf Mentions \\ \hline
    
    No overlapping involved & The left atrium is mildly dilated . & 1. \textbf{left atrium dilated} \\ \hline

    Overlapping involved, which accompany with coordination structure & I stopped it 8 weeks ago and still have much muscle pain and fatigue .  & 1. muscle pain; 2. \textbf{muscle fatigue} \\ 
    & & \\ \hline
    % & Then I sated having hip / leg / foot pain and numbness . & 1. \textbf{hip pain}; 2. \textbf{leg pain}; 3. foot pain; 4. numbness \\ 
     
    Overlapping involved, as well as irregular syntactic structure & Pain and cramping in my hands and lower legs . & 1. \textbf{Pain in my hands}; 2. \textbf{Pain in my lower legs}; 3. cramping in my hands; 4. \textbf{cramping in my lower legs} \\
    & & \\
    % & lots of pain in the muscles there , very tight . & 1. lots of pain in the muscles; 2. \textbf{muscles tight} \\
    \bottomrule
    \end{tabular}
    \caption{Examples involving discontiguous mentions, taken from CADEC and ShARe2013 data sets.~\label{table1-example}}
\end{table*}


==> table4-ablation.tex <==
\begin{table}[t]
\begin{small}
\setlength{\tabcolsep}{4pt} % Default value: 6pt
    \centering
    \begin{tabular}{ lc  c c c c c}
    \toprule
    && \multicolumn{2}{c}{\bf CADEC} && \multicolumn{2}{c}{\bf ShARe 2013} \\ \cmidrule{3-4}\cmidrule{6-7}
    \bf Model&& All & w. Disc. && All & w. Disc. \\ \cmidrule{1-1}\cmidrule{3-4}\cmidrule{6-7}
    Full && \bf 68.4 & \bf 65.4 && \bf 77.2 &  \bf 64.3 \\ 
    -Attention && 68.4 & 63.3 && 76.8 & 62.3 \\ 
    - ELMo && 66.7 & 62.2 && 75.2 & 60.9 \\ 
    BERT && 67.2 & 64.4 && 73.7 & 59.3 \\ \bottomrule
    \end{tabular}
    \caption{Ablation study to estimate the contribution of attention and pretrained contextual representations.~\label{table4-ablation}}
\end{small}
\end{table}

==> table6-evaluate-on-discontinuous-mentions.tex <==
\begin{table}
\begin{small}
\setlength{\tabcolsep}{2pt} % Default value: 6pt
    \centering
    \begin{tabular}{cr  cccc  cccc  cccc}
    \toprule
    &&& \multicolumn{3}{c}{\bf CADEC} && \multicolumn{3}{c}{\bf ShARe 2013} && \multicolumn{3}{c}{\bf ShARe 2014} \\ 
    \cmidrule{4-6}\cmidrule{8-10} \cmidrule{12-14}
    &\bf Model && P & R & F && P & R & F && P & R & F \\ 
    \cmidrule{2-2} \cmidrule{4-6}\cmidrule{8-10} \cmidrule{12-14}
    & Flat && 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ % 2019-Nov-11
    & BIO E. && 0 & 0 & 0 && 41.1 & 11.2 & 17.6 && 20.9 & 8.8 & 12.4 \\ % 2019-Nov-11
    & Graph && \bf 60.8 & 14.8 & 23.9 && \bf 79.1 & 37.3 & 50.7 && 45.8 & 40.1 & 42.7 \\ % 2019-Nov-11
    & Ours && 41.2 & \bf 35.1 & \bf 37.9 && 68.4 & \bf 43.3 & \bf 53.0 && \bf 49.8 & \bf 48.4 & \bf 49.1 \\ % 2019-Nov-11
    \bottomrule 
    \end{tabular}
    \caption{Evaluation results on discontinuous mentions.}
\end{small}
\end{table}
